SailCompass: Towards Reproducible and Robust Evaluation for Southeast Asian Languages

In this paper, we introduce SailCompass, a reproducible and robust evaluation benchmark for assessing Large Language Models (LLMs) on Southeast Asian Languages (SEA). SailCompass encompasses three main SEA languages, eight primary tasks including 14 datasets covering three task types (generation, multiple-choice questions, and classification). To improve the robustness of the evaluation approach, we explore different prompt configurations for multiple-choice questions and leverage calibrations to improve the faithfulness of classification tasks. With SailCompass, we derive the following findings: (1) SEA-specialized LLMs still outperform general LLMs, although the gap has narrowed; (2) A balanced language distribution is important for developing better SEA-specialized LLMs; (3) Advanced prompting techniques (e.g., calibration, perplexity-based ranking) are necessary to better utilize LLMs. All datasets and evaluation scripts are public.

==> tables/datasets.tex <==

\begin{table}[ht]
\begin{center}
\begin{tabular}{clllr}
\toprule
\bf Language & \bf Dataset & \bf Task & \bf Domain & \bf \# Examples \\
% \multicolumn{1}{c}{} &\multicolumn{1}{l}{}   &\multicolumn{1}{c}{}  &\multicolumn{1}{c}{} &\multicolumn{1}{r}{}    \\
\midrule
\multirow{7}{*}{Thai}         & XQuAD & QA & Wikipedia & 1,149 \\
 & Flores200 & MT & Wikipedia & 1,012 \\
 % & ThaiSum & TS & News & 3,671 \\
 & ThaiSum & TS & News & 1,000 \\
 & M3Exam & Exam & School materials & 2,163 \\
 & XNLI & NLI & Multi-genre & 5,010\\
 & XCOPA & CR & General & 500\\ 
 & BELEBELE & MRC & General & 900 \\ 
 & wisesight-sentiment & SA & Social media & 2,614\\
\midrule
\multirow{7}{*}{Indonesian}    & TyDiQA & QA  & Wikipedia & 565 \\
 & Flores200 & MT & Wikipedia & 1,012\\
 % & IndoSum & TS & News & 3,762\\
 & IndoSum & TS & News & 1,000\\
 % & IndoMT & MT & News & 2,000\\
 & M3Exam & Exam & School materials & 371 \\
 & IndoNLI & NLI & Multi-genre & 5,182 \\
 & XCOPA & CR & General & 500\\ 
 & BELEBELE & MRC & General & 900 \\
 & Indolem-sentiment & SA & Social media & 1,002  \\
 % & COPAL-ID & Commonsense & MCQ \\ 
\midrule
\multirow{7}{*}{Vietnamese}    & XQuAD & QA & Wikipedia & 1,169 \\
 & Flores200 & MT  & Wikipedia  & 1,012\\
 % & XLSum & TS & News & 2,676 \\
 & XLSum & TS & News & 1,000 \\
 & M3Exam & Exam & School materials & 1,789\\
 % & VMLU   & Exam & School materials & 744\\
 & XNLI & NLI  & Multi-genre & 5,010\\
 & XCOPA & CR & General & 500 \\ 
 & BELEBELE & MRC & General & 900 \\
 & VSMEC   & SA  & Social media & 692\\
 % & ViMMRC?   & Reading comprehension & - & - \\
\bottomrule
\end{tabular}
\end{center}
\caption{Our benchmark includes seven tasks: Question Answering (QA), Machine Translation (MT), Examination (Exam), Natural Language Inference (NLI), Commonsense Reasoning (CR), Machine Reading Comprehension (MRC), and Sentiment Analysis (SA). 
\longxu{Minimize this figure by spitting the dimensions to create `multi-index table'. Google it for a better illustration :) }
}
\label{dataset}
\end{table}

% \begin{table}[h]
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
%       & xquad & tydiqa & flores200 & thaisum & indosum & xlsum & xnli & indonli & xcopa & belebele & wisesight-sentimen & indolem-sentiment & vsmec \\ \hline
% thai  & \cellcolor[HTML]{FFFF99}1149 & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{FFFF99}1012 & \cellcolor[HTML]{FFFF99}1000 & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{FFFF99} & 5010 & \cellcolor[HTML]{FFFF99} & \cellcolor[HTML]{FFFF99}500 & \cellcolor[HTML]{FFFF99}900 & \cellcolor[HTML]{FFFF99}2614 & & \cellcolor[HTML]{C0C0C0} \\ \hline
% ind   & \cellcolor[HTML]{FFFF99}565  & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{FFFF99}1012 & \cellcolor[HTML]{FFFF99} & \cellcolor[HTML]{FFFF99}1000 & \cellcolor[HTML]{C0C0C0} & & \cellcolor[HTML]{FFFF99}5182 & \cellcolor[HTML]{FFFF99}500 & \cellcolor[HTML]{FFFF99}900 & & \cellcolor[HTML]{FFFF99}1002 & \cellcolor[HTML]{C0C0C0} \\ \hline
% vi    & \cellcolor[HTML]{FFFF99}1169 & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{FFFF99}1012 & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{FFFF99} & 5010 & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{FFFF99}500 & \cellcolor[HTML]{FFFF99}900 & & & \cellcolor[HTML]{FFFF99}692 \\ \hline
%       & \multicolumn{3}{c|}{wikipedia} & \multicolumn{2}{c|}{news} & news & multi-genre & multi-genre & general & general & social media & social media & social media \\ \hline
% \end{tabular}
% \caption{Data summary for different languages and tasks}
% \label{table:data_summary}
% \end{table}


==> tables/exam.tex <==
\begin{table}[ht]
\begin{center}
\scalebox{0.9}{
\begin{tabular}{crrr}
\toprule
\multirow{2}{*}{\bf Model}  & \multicolumn{3}{c}{\bf EXAM} \\
% \cline{2-3}
& Thai (ppl/gen) & Javanese (ppl/gen) & Vietnamese (ppl/gen) \\
\midrule
\texttt{Llama-3-8B} &  30.84 / 38.27 & 35.04 / 39.94 & 42.76 / 53.55 \\
\texttt{Mistral-7B} & 26.03 / 31.00 & 28.03 / 29.59 & 36.11 / 43.54\\
\texttt{Gemma-7B} & 28.20 / 35.04 & 29.92 / 40.73 & 48.57 / 60.65 \\
\texttt{Typhoon-8B} & 31.90 / 34.23 & 30.46 / 47.34 & 34.77 / 43.21\\
\texttt{VinaLLaMA-7B} & 22.65 / 26.42 & 21.56 / 14.42 & 36.22 / 36.95 \\
\texttt{BLOOM-7B1} & 23.35 / 23.45 & 28.30 / 21.27 & 38.07 / 26.50 \\
\texttt{Sailor-7B} & 30.00 / 35.85 & 32.88 / 38.33 & 44.10 / 51.98\\
\texttt{SeaLLM-7B} & 27.23 / 24.26 & 25.61 / 26.26 & 36.44 / 38.85 \\
\texttt{Sea-Lion-7B} & 25.29 / 21.56 & 22.64 / 23.90 & 38.74 / 26.89\\
\midrule
\end{tabular}
}
\end{center}
\caption{Main results on the EXAM task (ppl).}
\label{m3_ppl}
\end{table}




























==> tables/pre_gen.tex <==
\begin{table}[ht]
\begin{center}
\scalebox{0.85}{
\begin{tabular}{ccrrrr}
\toprule
\bf Language & \bf Model & \bf QA & \bf MT (En \!\Arrow{.2cm}\!\! X) & \bf MT (X \!\Arrow{.2cm}\!\! En) & \bf TS  \\
\midrule
\multirow{3}{*}{Thai} & \texttt{Sea-Lion-7B} & 43.52 & 7.15 & 20.81 & 22.77  \\
&  \texttt{SeaLLM-7B} & 49.70 & 8.01 & 24.08 & 17.98 \\
&  \texttt{Sailor-7B} & \bf 57.88 & \bf 10.01 & \bf 28.82 & 26.84 \\
\midrule
\multirow{3}{*}{Indonesian} & \texttt{Sea-Lion-7B} & 50.09 & 32.49 & 32.33 & 30.22 \\
&  \texttt{SeaLLM-7B} & 50.62 & 36.01 & 38.81 & 42.19 \\
&  \texttt{Sailor-7B} & \bf 60.53 & \bf 41.40 & \bf 41.11 & 45.42 \\
\midrule
\multirow{3}{*}{Vietnamese} & \texttt{Sea-Lion-7B} & 42.43 & 35.59 & 27.32 &  \\
&  \texttt{SeaLLM-7B} & 49.62 & 35.64 & 30.49 & 4.58 \\
&  \texttt{Sailor-7B} & \bf 53.81 & \bf 39.73 & \bf 34.62 & 5.48\\
\bottomrule
\end{tabular}
}
\end{center}
\caption{Main evaluation results on generation tasks.}
\label{main_results_gen}
\end{table}

==> tables/pre_mcq.tex <==
\begin{table}[ht]
\begin{center}
\scalebox{0.85}{
\begin{tabular}{ccrrrrr}
\toprule
\bf Language & \bf Model & \bf Exam & \bf NLI & \bf CR & \bf MRC & \bf SA \\
\midrule
\multirow{3}{*}{Thai} & \texttt{Sea-Lion-7B} & 25.29 & 33.33 & \bf 60.80 & 36.33 & \bf 29.15 \\
&  \texttt{SeaLLM-7B} & 27.18 & 33.33 & 58.20 & 37.78 & 18.44 \\
&  \texttt{Sailor-7B} & \bf 30.00 & \bf 34.57 & 59.00 & \bf 41.56 & 18.52\\
\midrule
\multirow{3}{*}{Indonesian} & \texttt{Sea-Lion-7B} & 22.91 & 34.00 & 60.60 & 35.56 & 73.55\\
&  \texttt{SeaLLM-7B} & 26.95 & \bf 34.56 & 71.6 & 43.11 & 74.25  \\
&  \texttt{Sailor-7B} & \bf 32.88 & 34.16 & \bf 72.20 & \bf 44.33 & \bf 82.63\\
\midrule
\multirow{3}{*}{Vietnamese} & \texttt{Sea-Lion-7B} & 38.74 & 33.43 & 67.80 & 37.00 & 19.08 \\
&  \texttt{SeaLLM-7B} & 36.50 & 33.33 & 67.60 & 43.00 & \bf 32.80  \\
&  \texttt{Sailor-7B} & \bf 44.10 & \bf 34.03 & \bf 72.20 & \bf 45.33 & 18.06\\
\bottomrule
\end{tabular}
}
\end{center}
\caption{Main evaluation results on MCQ tasks.}
\label{main_results_mcq}
\end{table}


==> tables/sailor_mmlu.tex <==
\begin{table}[ht]
\begin{center}
\begin{tabular}{lcc}
\toprule
\multicolumn{1}{c}{\bf Model}  &\multicolumn{1}{c}{${\bm{S_a}}_{_{PPL}}$} &\multicolumn{1}{c}{${\bm{I_oS_oI_a}}_{_{PPL}}$} \\
\midrule
\verb|Sailor-7B|   & 42.56 &  62.56  \\
\verb|Sailor-7B (Manipulated)|   & 41.78 & 73.33\\
\bottomrule
\end{tabular}
\end{center}
\caption{Performance comparison with the manipulated training on the BELEBELE (th) benchmark.}
\label{sailor_mmlu}
\end{table}
